Fairness Through Robustness: Investigating Robustness Disparity in Deep Learning

Deep neural networks (DNNs) are increasingly used in real-world applications (e.g. facial recognition). This has resulted in concerns about the fairness of decisions made by these models. Various notions and measures of fairness have been proposed to ensure that a decision-making system does not disproportionately harm (or benefit) particular subgroups of the population. In this paper, we argue that traditional notions of fairness that are only based on models' outputs are not sufficient when the model is vulnerable to adversarial attacks. We argue that in some cases, it may be easier for an attacker to target a particular subgroup, resulting in a form of \textit{robustness bias}. We show that measuring robustness bias is a challenging task for DNNs and propose two methods to measure this form of bias. We then conduct an empirical study on state-of-the-art neural networks on commonly used real-world datasets such as CIFAR-10, CIFAR-100, Adience, and UTKFace and show that in almost all cases there are subgroups (in some cases based on sensitive attributes like race, gender, etc) which are less robust and are thus at a disadvantage. We argue that this kind of bias arises due to both the data distribution and the highly complex nature of the learned decision boundary in the case of DNNs, thus making mitigation of such biases a non-trivial task. Our results show that robustness bias is an important criterion to consider while auditing real-world systems that rely on DNNs for decision making. Code to reproduce all our results can be found here: \url{https://github.com/nvedant07/Fairness-Through-Robustness}

==> lower_bounds.tex <==
\section{An Alternate Robustness Measure: Robustness Certificates}\label{sec:lower_bounds}

In section~\ref{sec:robustness_bias} we argued that a key element to measure robustness bias is the distance of each point from the decision boundary, $d_\theta(x)$. For modern-day classifiers (\ie~Deep Neural Networks), exactly computing this distance is challenging since the decision boundary is a non-convex function, hence we used distance from adversarial samples as an upper bound in section~\ref{subsec:upper_bounds} to estimate this distance. In this section we explore an alternative approach that measures a lower bound on the distance. We borrow from recent work on training provably robust classifiers~\cite{salman2019provable, singla2020curvature, cohen2019smoothing}. 

One key component of these works is to ``certify'' each input $x$, \ie, for each input these methods calculate a radius in which the prediction of $x$ will not change. We use the methodology proposed by Salman et al.~\cite{salman2019provable} since it scales to larger and deeper neural networks and is state-of-the-art in provable defenses. They use \textit{randomized smoothing} to transform $f$ to a new smooth classifier $g$. This new classifier $g$ is more robust to perturbations while also having accuracy similar to the original model. It's also possible to calculate the radius $\delta$ ($\ell_2$ distance) in which a given input's ($x$) prediction remains the same for the smoothed classifier. A given input $x$ is then said to be provably robust for a $\delta$ $\ell_2$-perturbation where $\delta$ is the robustness certificate of $x$.

For each point we use its $\delta$, calculated using the method proposed by~\cite{salman2019provable}, as a proxy for $d_{\theta}(x)$. The magnitude of $\delta$ for an input is a measure of how robust an input is. Inputs with higher $\delta$ are more robust than inputs with smaller $\delta$. Thus, we want to study 2 things:
\begin{enumerate}
    \item Do models exhibit robustness bias when $d_\theta(x)$ is estimated using~\cite{salman2019provable}?
    \item Are the trends in robustness bias similar to the trends reported for upper bounds using adversarial samples in section~\ref{sec:experiments}?
\end{enumerate}

\subsection{Experiments using Robustness Certificates}\label{sec:lower_bounds_experiments}

Figure~\ref{fig:lb_adience},~\ref{fig:lb_utkface_race},~\ref{fig:lb_utkface_gender},~\ref{fig:lb_cifar10},~\ref{fig:lb_cifar100},~\ref{fig:lb_cifar100super} show the trend for robustness certificates for Adience, UTKFace paritioned by race, UTKFace partitioned by gender, CIFAR-10, CIFAR-100 and CIFAR-100 (super classes only) respectively. The trend is similar to the trend observed with upper bounds in Section~\ref{sec:experiments}. \todo{Elaborate here.}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/utkface_race/utkface_classifier_output_race_lbs.pdf}
        \caption{Deep CNN}
        \label{fig:lb_utkface_race_deep_cnn}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{lb_plots/utkface_race/densenet_output_race_lbs.pdf}
        \caption{Densenet}
        \label{fig:lb_utkface_race_densenet}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/utkface_race/resnet_output_race_lbs.pdf}
        \caption{Resnet-50}
        \label{fig:lb_utkface_race_resnet}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/utkface_race/vgg_output_race_lbs.pdf}
        \caption{VGG-19}
        \label{fig:lb_utkface_race_vgg}
    \end{subfigure}
    
\caption{ [Robustness Certificates] UTKFace partitioned by race.
} 
\label{fig:lb_utkface_race}
\end{figure}


\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/utkface_gender/utkface_classifier_output_gender_lbs.pdf}
        \caption{Deep CNN}
        \label{fig:lb_utkface_gender_deep_cnn}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{lb_plots/utkface_gender/densenet_output_gender_lbs.pdf}
        \caption{Densenet}
        \label{fig:lb_utkface_gender_densenet}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/utkface_gender/resnet_output_gender_lbs.pdf}
        \caption{Resnet-50}
        \label{fig:lb_utkface_gender_resnet}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/utkface_gender/vgg_output_gender_lbs.pdf}
        \caption{VGG-19}
        \label{fig:lb_utkface_gender_vgg}
    \end{subfigure}
    
\caption{ [Robustness Certificates] UTKFace partitioned by gender.
} 
\label{fig:lb_utkface_gender}
\end{figure}


\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/adience/adience_classifier_output_gender_lbs.pdf}
        \caption{Deep CNN}
        \label{fig:lb_adience_deep_cnn}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/adience/densenet_output_gender_lbs.pdf}
        \caption{Densenet}
        \label{fig:lb_adience_densenet}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/adience/resnet_output_gender_lbs.pdf}
        \caption{Resnet-50}
        \label{fig:lb_adience_resnet}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/adience/vgg_output_gender_lbs.pdf}
        \caption{VGG-19}
        \label{fig:lb_adience_vgg}
    \end{subfigure}
    
\caption{ [Robustness Certificates] Adience partitioned by gender.
} 
\label{fig:lb_adience}
\end{figure}


\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/cifar10/output_deep_cnn_label_lbs.pdf}
        \caption{Deep CNN}
        \label{fig:lb_cifar10_deep_cnn}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/cifar10/output_pyramidnet_label_lbs.pdf}
        \caption{Pyramidnet, $\alpha$ = 64, depth = 110}
        \label{fig:lb_cifar10_pyramidnet}
    \end{subfigure}
    
\caption{ [Robustness Certificates] CIFAR-10 partitioned by class labels.
} 
\label{fig:lb_cifar10}
\end{figure}


\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/cifar100/output_deep_cnn_cifar100_label_lbs.pdf}
        \caption{Deep CNN}
        \label{fig:lb_cifar100_deep_cnn}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/cifar100/output_pyramidnet_label_lbs.pdf}
        \caption{Pyramidnet (Bottleneck), $\alpha$ = 48, depth = 164}
        \label{fig:lb_cifar100_pyramidnet}
    \end{subfigure}
    
\caption{ [Robustness Certificates] CIFAR-100 partitioned by class labels.
} 
\label{fig:lb_cifar100}
\end{figure}


\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/cifar100super/output_deep_cnn_cifar100_label_lbs.pdf}
        \caption{Deep CNN}
        \label{fig:lb_cifar100super_deep_cnn}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{adversarial fairness - NeurIPS/lb_plots/cifar100super/output_pyramidnet_label_lbs.pdf}
        \caption{Pyramidnet (Bottleneck), $\alpha$ = 48, depth = 164}
        \label{fig:lb_cifar100super_pyramidnet}
    \end{subfigure}
    
\caption{ [Robustness Certificates] CIFAR-100 (only super classes) partitioned by class labels.
} 
\label{fig:lb_cifar100super}
\end{figure}

\subsection{Comparison of Robustness Certificates and Upper Bounds}\label{sec:lower_bounds_experiments}

We present the percent agreement in the signedness of $\sigma^{\text{RS}}$ with $\sigma^{\text{DF}}$ and the signedness of $\sigma^{\text{RS}}$ with $\sigma^{\text{CW}}$. These results are presented in Table \ref{RS-DF-CW}.

\begin{table}[h]
\centering
\caption{Percentage of agreement with $\sigma^{\text{RS}}$ and $\sigma^{\text{DF}}$ and $\sigma^{\text{CW}}$}
\label{RS-DF-CW}
\begin{tabular}{l|cc}
\hline

        & DeepFool          & CarliniWagner  \\
\midrule
Adience & 83.33 & 79.63\\
UTKFace & 74.24 & 72.73\\
CIFAR10 & 75.00 & 76.67\\
CIFAR100 & 53.83 & 54.00\\
CIFAR100super & 65.83 & 66.67\\
\bottomrule
\end{tabular}
\end{table}



==> new_adverm.tex <==
\section{New \AdvERM{}}\label{sec:new_regularization}

Re-formulation of \AdvERM{} which also adds terms for increased robustness.

\vspace{-2.5mm}
{\small
\begin{multline*}
    \tilde{\RBmeasure}{(P,\tau)} = \left|  \frac{1}{\displaystyle \sum_{x\notin P} \mathbbm{1}\{ y = \yhat \}} \sum_{\substack{x \notin P\\y = \yhat}} \mathbbm{1}\{ d_\theta(x) > \tau \}  - \frac{1}{\displaystyle\sum_{x\in P} \mathbbm{1}\{ y = \yhat \}} \sum_{\substack{x \in P\\y = \yhat}} \mathbbm{1}\{ d_\theta(x) > \tau \}  \right| \, + \, \\ 
    \frac{1}{\displaystyle \sum_{x\notin P} \mathbbm{1}\{ y = \yhat \}} \sum_{\substack{x \notin P\\y = \yhat}}\mathbbm{1}\{ d_\theta(x) < \tau \} \, + \, \\
    \frac{1}{\displaystyle\sum_{x\in P} \mathbbm{1}\{ y = \yhat \}} \sum_{\substack{x \in P\\y = \yhat}} \mathbbm{1}\{ d_\theta(x) < \tau \}
\end{multline*}
}

==> regularization_formulation.tex <==
\section{Reducing Robustness Bias through Regularization}\label{sec:regularization}
Motivated by evidence (see Section \ref{sec:experiments}) that robustness bias exists in a diverse set of real-world models and datasets, we will now show that the expression of robustness bias can be included in an optimization. We do so in a natural way: by formulating a regularization term that captures robustness bias.
 
Recall the traditional Empirical Risk Minimization objective, $\ERM{} := l_{cls} (f_\theta(X), Y)$ where $l_{cls}$ is cross entropy loss. Now we wish to model our measure of fairness (see Section \ref{sec:robustness_bias}) and minimize for it alongside $\ERM{}$. We first write the empiric estimate of $\RBmeasure{(P,\tau)}$ as $\tilde{\RBmeasure}{(P,\tau)}$; a full derivation can be found in \Cref{app:regularizer-derivation}.  Formally,
\vspace{-2.5mm}
{\small
\begin{equation*}
    \tilde{\RBmeasure}{(P,\tau)} = \left|  \frac{1}{\displaystyle \sum_{x\notin P} \mathbbm{1}\{ y = \yhat \}} \sum_{\substack{x \notin P\\y = \yhat}} \mathbbm{1}\{ d_\theta(x) > \tau \}  - \frac{1}{\displaystyle\sum_{x\in P} \mathbbm{1}\{ y = \yhat \}} \sum_{\substack{x \in P\\y = \yhat}} \mathbbm{1}\{ d_\theta(x) > \tau \}  \right|
\end{equation*}

}
\vspace{-3mm}



To use this as a regularizer during training, we must compute the closed form expression of $d_\theta$. For this, we take inspiration from the way adversarial inputs are created using DeepFool~\cite{moosavi2016deepfool}. Just like in DeepFool, we also approximate distance from $f_\theta$ considering $f_\theta$ to be linear (even though it may be a highly non-linear DNN). There, we incorporate into $\tilde{\RBmeasure}{(P,\tau)}$ the approximation $d_\theta(x) = \, | \,  \frac{f_\theta(x)}{|| \nabla_x f_\theta(x) ||}  \, | \,$.  Finally, we minimize for the new objective function, $\AdvERM{} := l_{cls} (f_\theta(X), Y) + \alpha  \RBmeasure{(P,\tau)}$.

\subsection{Experimental Results using Regularized Models}


\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{regularized_plots/cifar10/deep_cnn/inv_cdf_truck.pdf}
        \caption{CIFAR10 (no reg.)}
        \label{fig:cifar10_truck_main_paper}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{regularized_plots/cifar10/deep_cnn/regularized_truck/RegularizedLoss_probabilities_exact_alpha_01_tau_50_inv_cdf.pdf}
        \caption{$\alpha = 0.1$, $\tau = 5.0$.}
        \label{fig:cifar10_truck_reg_alpha_0.1_tau_5.0}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{regularized_plots/utkface_race/utkface_classifier/inv_cdf_Black.pdf}
        \caption{UTKFace (no reg.)}
        \label{fig:utkface_race}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=1\textwidth]{regularized_plots/utkface_race/utkface_classifier/regularized/RegularizedLoss_probabilities_exact_alpha_10_tau_50_inv_cdf.pdf}
        \caption{$\alpha = 1.0$, $\tau = 5.0$.}
        \label{fig:utkface_race_alpha_1.0_tau_5.0}
    \end{subfigure}
\caption{In the unregularized model, ``truck'' in CIFAR10 tends to be more robust than other classes (\ref{fig:cifar10_truck_main_paper}); however, using \AdvERM{} reduces that disparity (\ref{fig:cifar10_truck_reg_alpha_0.1_tau_5.0}).  We see similar behavior for UTKFace (\ref{fig:utkface_race} \& \ref{fig:utkface_race_alpha_1.0_tau_5.0}). 
} 
\label{fig:regularized_cifar}
\end{figure}

Using our regularized objective, \AdvERM{}, we re-train the model (details in Appendix~\ref{app:regularizer}) considering $\alpha$ and $\tau$ as hyperparameters, in addition to the traditional hyperparameters such as learning rate, momentum etc (see \Cref{app:regularizer} for reproducibility details). Here, we evaluate the regularized model, after training for a number of vaues of $\alpha$ and $\tau$, for CIFAR10 considering each class as the partition $\mathcal{P}$, and UTKFace with the sensitive attribute race as a partition $\mathcal{P}$.
Figure~\ref{fig:regularized_cifar} shows example results for the regularized models for the class ``truck'' in CIFAR10 and for the class ``black'' in UTKFace. Results for additional classes, datasets, and models can be found in~\Cref{app:regularizer-experiments}.

Across the two datasets, we see that for an appropriate $\alpha$ and $\tau$, we are able to reduce the robustness disparity---\ie, difference between blue and red curves---that existed in the original model. For these two datasets, this does not come at any cost of accuracy. We observe test set accuracy of $86.97\%$ on CIFAR10 without regularization and $87.82\%$ with regularization. Similarly for UTKFace we see accuracies of $66.25\%$ and $65.52\%$ for no regularization and with regularization respectively. Results for other models and hyperparameters can be found in Appendix~\ref{app:regularizer-experiments}. We interpret our experiments as an indication that an optimization-based approach can play a part in a larger robustness bias-mitigation strategy, rather than serving as panacea. 
